Preserved central model for faster bidirectional compression in distributed settings

We develop a new approach to tackle communication constraints in a distributed learning problem with a central server. We propose and analyze a new algorithm that performs bidirectional compression and achieves the same convergence rate as algorithms using only uplink (from the local workers to the central server) compression. To obtain this improvement, we design MCM, an algorithm such that the downlink compression only impacts local models, while the global model is preserved. As a result, and contrary to previous works, the gradients on local servers are computed on perturbed models. Consequently, convergence proofs are more challenging and require a precise control of this perturbation. To ensure it, MCM additionally combines model compression with a memory mechanism. This analysis opens new doors, e.g. incorporating worker dependent randomized-models and partial participation.

==> extensions.tex <==
\section{Todo}
\begin{enumerate}
    \item Etendre la preuve de convergence a non iid 
    \item Etendre la preuve de convergence au bruit en $w_*$
    \item Cas non-convex. La coco ne tient plus, comment minorer le produit scalaire $2\gamma \PdtScl{truc}{truc2}$ et comment gérer la norme au carré ?
    \item Expérience en réseau de neuronnes (MNIST). On pourrait faire un 3 layer.
    \item 
\end{enumerate}

\subsection{Non-iid}
The next assumptions is used to quantify the heterogeneity between worker's datasets.
\begin{assumption}[Bounded gradient at $w_*$]
\label{asu:bounded_noises_across_devices}
There exists a constant $B \in \mathbb{R_+}$, s.t.: 
\gs
\[
%\forall i \in \llbracket 1, N \rrbracket\,, \quad
\frac{1}{N} \sum_{i=0}^N \| \nabla F_i(w_*)\|^2 \leq B^2\,.
\gs\] 
\end{assumption}
\gs
Combining \Cref{asu:noise_sto_grad,asu:bounded_noises_across_devices} results in an upper bound on the averaged squared norm of stochastic gradients at $w_*$: for all $k$ in $\N$, a.s.,
%for all $i$ in $\llbracket 1, N \rrbracket$:
%\forall k \in \N, \forall i \in \llbracket 1, N \rrbracket\,, \quad 
$$\frac{1}{N} \sum_{i=1}^N\Expec{\|\gwkstar^i\|^2}{\Fdwncomp_{k}} \leq \ffrac{\sigmstar^2}{b} + B^2 \,. $$
%\end{align} 


\subsection{Extension to nois at optimum}

Below, we introduce cocoercivity (see \citet{zhu_co-coercivity_1996} for more details about this hypothesis). This assumption (see implies that all $(F_i)_{i \in \llbracket 1, N \rrbracket}$ are $L$-smooth. In machine learning framework, this is for example valid for both Least Squares Regression (LSR) and Logistic Regression (LR)~\citep{patel_communication_2019}. 
\begin{assumption}[Cocoercivity of stochastic gradients (in quadratic mean)]
\label{asu:cocoercivity}
  We suppose that for all $k$ in $\N$,  stochastic gradients functions $(\g_k^i)_{i \in \llbracket1, N \rrbracket}$ are  L-cocoercive in quadratic mean. That is, for  $k$ in $\N$,   $i$ in $\llbracket1, N \rrbracket$ and for all vectors $w_1, w_2$ in $\WW$, we have:
  \begin{align*}
\E [ \| \g^i_{k}(w_1) - \g_{k}^i(w_2) \|^2 ] \leq &\\
  & \hspace{-3em} L  \PdtScl{\nabla F_i (w_1) - \nabla F_i(w_2)}{w_1 - w_2} \,.
  \end{align*}
\end{assumption}
\gs\gs
E.g., this is  true under the much stronger assumption that  stochastic gradients functions $(\g_k^i)_{i \in \llbracket1, N \rrbracket}$ are \textit{almost surely} $L$-cocoercive, i.e.: 
  $  \| \g^i_{k}(w_1) - \g_{k}^i(w_2) \|^2 \leq L \PdtScl{\g^i_{k}(w_1) - \g_{k}^i(w_2)}{w_1 - w_2} \,$.
  
  \subsection{Unifying assumptiom}
  \begin{assumption}
\label{asu:link_omega_gradients}
For $k$ in $\N$, there exists a sequence $(\theta^k_{k-i})_{i=1}^k$ and a constant $\theta$ such that for any algorithm encompassed by \Cref{algo} we have almost surely:
\begin{align*}
    &\Expec{\SqrdNrm{w_k - \widehat{w}_k}}{w_k} \leq \gamma^2 \omgC^\dwn \theta \ffrac{\sigma^2}{b} \\
    &\qqquad + \gamma^2 \omgC^\dwn \sum_{i=0}^k \theta^k_{k-i} \E \SqrdNrm{\nabla F(\widehat{w}_{i-1})}\,.
\end{align*}
\end{assumption}

  
  
  \subsection{Other points}
  
  
  \begin{assumption}[Convexity]
\label{asu:strongcvx}
$F$ is convex, that is for all vectors $w_1, w_2$ in $\WW$:
\begin{align*}
%\forall w,_1 w_2 \in \WW\,, \quad
F(w_2) \geq F(w_1) + \PdtScl{\nabla F(w_1)}{w_2 - w_1} \,.
\end{align*}
\end{assumption}



\section{faire une description de toutes les techniques de preuves}


\section{The framework for randomization}
\label{sect:framework_randomization}
In this section, we present the framework developed for bidirectional compression.

For $k \in \N$ and $i \in \llbracket 1, N \rrbracket$, we denote with $\Delta_k^i$ (resp. $\Omega_k^i$), the value that is going to be communicated from local device $i$ to central server at iteration $k$ (resp. from central server to local device $i$). And we note $\widehat{\Delta}_k^i$ and $\widehat{\Omega}_k^i$ the vectors after having been compressed by the up operator $\C^\dwn_i$ and the down operator $\C\up_i$:
\begin{align}
\label{eq:def_delta_omega}
\begin{split}
    \widehat{\Delta}_k^i &= \C_i^{\up} ( \g_{k+1}^i(\widehat{\Omega}_k^i + H_k^i) - h_k^i + e_k^i) \,, \\
    \widehat{\Omega}_k^i &= \C_i^{\dwn} ( X_{k+1} - H_k^i + E_k^i) \,. \\
\end{split}
\end{align}
$X_{k+1}$ is the \textit{valuable information} that we want to communicate to local nodes, either we send back the new model and then $X_{k+1} = w_k - \ffrac{\gamma}{N} \sum_{i=1}^N \widehat{\Delta}_k^i + h_k^i$, either we send back the average gradient and then $X_{k+1} = \frac{1}{N} \sum_{i=1}^N \widehat{\Delta}_k^i + h_k^i$. This work is the first to define the notion of \textit{randomization} in the context of compression. The algorithm is said to be randomized if the master node carry out a new compression for each worker, which thus receive a potentially unique vector. All existing algorithms do not using randomization and consequently verify : $\forall i, j \in \llbracket 1, N \rrbracket^2, \C_i^\dwn(\cdot) = \C_j^\dwn(\cdot)$.

The error-feedback and the memory mechanisms are controlled with the following equations:
\begin{align}
\label{eq:def_ef}
\begin{split}
    e_k^{i+1} = \Delta_k^i - \widehat{\Delta}_k^i \qquad &\text{and} \quad E_k^{i+1} = \Omega_k^i - \widehat{\Omega}_k^i \,,\\
    h_k^{i+1} = h_k^i + \alpha \widehat{\Delta}_k^i \qquad &\text{and} \quad H_k^{i+1} = H_k^i + \alpha \widehat{\Omega}_k^i \,.
\end{split}
\end{align}

To update the model, we need to adjust \Cref{eq:sgd_statement}. There are two choices, either we update the model with the information compressed twice (\textit{the degraded update}), either with the values compressed once (before compressing for the down communication, this is \textit{the non-degraded update}).
\begin{enumerate}
    \item The degraded update corresponds to $w_{k+1} = w_k - \ffrac{\gamma}{N}\sum_{i=1}^N \widehat{\Omega}_k^i + H_k^i$ if we compress the gradients, and to $w_{k+1} = \frac{1}{N} \sum_\iN \widehat{\Omega}_k^i + H_k^i$ if we compress the model. All compression $\widehat{\Omega}_k^i$ have been compressed.
    \item The non-degraded update corresponds to $w_{k+1} = w_k - \gamma X_{k+1}$ if we compress the gradients, and to $w_{k+1} = X_{k+1}$ if we compress the model. In other words, we use the valuable information that will later be compressed to update the global model.
\end{enumerate}

In particular, this framework recovers \Diana, \DoubleSqueeze, \Artemis, \Dore~(the variant without regularization) and more algorithms. The settings of the most popular algorithms within this framework are summarized in \Cref{tab:algo_summary}. 

\section{Experiments}

- Toy logistic en dimension beaucoucp

- une expe en NN



\section{Illustration }
dans la partie de la variance réduite pour \RMCM


\section{Proofs}
\aymeric{todo: check it Proposition below can be improved with $||g_k||$}



\section{TODO}

section 4.3

faire preuve quadratique

cas non convexe




==> proof_ghost_heterog.tex <==

\subsection{Proofs for \ghost}
\label{app:subsec:proof_for_ghost_with_up_mem}

In the case of heterogeneous worker, the definition of \ghost~must be updated.
\begin{definition}[\ghost~algorithm with heterogeneous worker]
\label{app:def:ghost_heterog}
The \ghost~algorithm is defined as follows, for $k \in \N$, for all $i \in \llbracket 1, N \rrbracket$ we have:
\begin{align}
\label{app:eq:ghost_heterog}
          w_{k+1} = w_k - \gamma \ffrac{1}{N} \sum_{i=1}^N \widehat{\Delta}_{k+1}^i \text{\quad and\quad} \widehat{w}_{k+1} = w_k - \gamma \C^{\dwn} \left(\ffrac{1}{N} \sum_{i=1}^N \widehat{\Delta}_{k+1}^i \right) \,,
\end{align}
with $\Delta_{k}^i = \g_{k+1}^i(\widehat{w}_{k}) - h_k^i $ and $h_{k+1}^{i} = h_k^i + \alpha\up \C\up({\Delta}_k^i)$.
\end{definition}

\subsubsection{Control of the Variance of the local model for \ghost}
\label{app:subsec:prop_ghost_assumption_heterog}

The proof of \Cref{app:prop:ghost_contraction} is straightforward using \Cref{def:ghost} that defines the \ghost~algorithm. 
\begin{theorem}
\label{app:prop:ghost_variance_heterog}
Consider the \ghost~update in \cref{eq:ghost}, under \Cref{asu:expec_quantization_operator,asu:smooth,asu:noise_sto_grad}, for all $k$ in $\N$ with the convention $\nabla F(w_{-1}) = 0$:
\begin{align*}
    \Expec{\SqrdNrm{w_k - \widehat{w}_k}}{\wkmhat} &\leq \bigpar{1 + \frac{4\omgC\up }{N}} \gamma^2 L \omgC\dwn \Expec{\PdtScl{\nabla F(\wkmhat)}{\wkmhat - w_*}}{\wkmhat} \\
    &\qquad + 2\omgC\up \omgC\dwn \gamma^2\Expec{\upMemTerm_{k-1}}{\wkmhat} \\
    &\quad+ \frac{\gamma^2 \omgC\dwn \sigma^2}{Nb} (1 + 4 \omgC\up)  \,.
\end{align*}
\end{theorem}

\begin{proof}
Let $k$ in $\N$, by \Cref{def:ghost} we have:
\begin{align*}
    \SqrdNrm{w_k - \widehat{w}_k} &= \left\| \bigpar{\wkm - \ffrac{\gamma}{N} \sum_{i=1}^N \C\up(\Delta_{k-1}^i) + h_{k-1}^i} \right. \\
    & \qquad \left.- \bigpar{\wkm - \gamma \C\dwn \bigpar{\ffrac{1}{N} \sum_{i=1}^N \C\up(\Delta_{k-1}^i) + h_{k-1}^i }} \right\|^2 \\
    &= \gamma^2 \SqrdNrm{\C\dwn \bigpar{\ffrac{1}{N} \sum_{i=1}^N \C\up(\Delta_{k-1}^i) + h_{k-1}^i } - \bigpar{\ffrac{1}{N} \sum_{i=1}^N \C\up(\Delta_{k-1}^i) + h_{k-1}^i}} \,.
\end{align*}

Taking expectation w.r.t. downlink compression, as $\ffrac{1}{N} \sum_{i=1}^N \C\up(\Delta_{k-1}^i) + h_{k-1}^i $ is $\wkm$-measurable:
\begin{align*}
    \Expec{\SqrdNrm{w_k - \widehat{w}_k}}{\wkm} &= \gamma^2 \omgC\dwn \Expec{\SqrdNrm{\ffrac{1}{N} \sum_{i=1}^N \C\up(\Delta_{k-1}^i) + h_{k-1}^i }}{\wkm} = \gamma^2 \omgC\dwn \SqrdNrm{\gwkHAT} \,,
\end{align*}

and \Cref{app:lem:grad_sto_to_grad_heterog} allows to upper bound $\Expec{\SqrdNrm{\gwkHAT}}{\wkmhat}$.
\end{proof}



\subsubsection{Convergence of \ghost}
\label{app:subsec:proof_thms_ghost_heterog}

In this subsection, we give the proof of \Cref{app:thm:contraction_ghost,app:thm:cvgce_ghost} in the case of heterogeneous workers.

\fbox{
\begin{minipage}{\textwidth}
\begin{theorem}[Convergence of \ghost, convex case]
\label{app:thm:cvgce_ghost_heterog}
Under \Cref{asu:cvx_or_strongcvx,asu:expec_quantization_operator,asu:smooth,asu:noise_sto_grad} with $\mu=0$ (convex case), with a learning rate such that $\alpha\up (1 + \omgC\up) \leq 1$, taking a step size s.t.:
$$
\gamma L \leq \min \bigg\{ \ffrac{1}{16 \TTwo \omgC\up /N}, \ffrac{1}{4 \bigpar{1 + \ffrac{4 \omgC\up}{ N}}}, \ffrac{1}{2 \sqrt{2 \omgC\dwn \bigpar{1 + \frac{4\omgC\up }{N}}}}, \ffrac{1}{4\sqrt{2 \omgC\dwn \frac{\omgC\up}{N}}} \bigg\} \,
$$ 
for any $k$ in $\N$, defining:
$$V_k := \FullExpec{\SqrdNrm{w_k - w_*}} + \ffrac{\gamma}{2}\FullExpec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}} +  \gamma^2 \cst_1 \FullExpec{\upMemTerm_{k-1}} + \gamma^3 L \cst_2 \FullExpec{\upMemTerm_{k-2}}\,,$$
with $\cst_1 = \ffrac{2 \omgC\up}{\TTwo}$, $\cst_2 = \ffrac{4 \omgC\dwn \omgC\up}{\TOne}$, we have: 
\begin{align*}
V_k \leq V_{k-1} - \gamma \FullExpec{F(\wkm) - F(w_*)} + \frac{\gamma^2 \sigma^2 \Phi^{\Gheterog}(\gamma)}{Nb}\,,
\end{align*}
with $\Phi^{\Gheterog}(\gamma) := \bigpar{1+8\omgC\up} \bigpar{1 + 2 \gamma L \omgC\dwn}$.

\end{theorem}
\end{minipage}
}

\begin{proof}

We denote for $k$ in $\N^*$ $\gwktilde = \ffrac{1}{N} \sum_\iN \widehat{\Delta}_{k-1}^i + h_{k-1}^i$ with $\Delta_{k-1}^i = \gwkihat - h_{k-1}^i$, and $\upMemTerm_k = \frac{1}{N^2} \sum_\iN \Expec{\SqrdNrm{h_{k}^i - \nabla F_i(w_*)}}{\wkmhat}$.

Let $k$ in $\N^*$, by definition:
\begin{align*}
    \SqrdNrm{w_k - w_*} \leq \SqrdNrm{\wkm - w_*} - 2\gamma \PdtScl{\gwkHAT}{\wkm - w_*} + \gamma^2 \SqrdNrm{\gwkHAT} \,.
\end{align*}
Next, we expend the inner product as following:
\begin{align*}
    \SqrdNrm{w_k - w_*} \leq \SqrdNrm{\wkm - w_*} - 2\gamma \PdtScl{\gwkHAT}{\wkmhat - w_*} - 2\gamma \PdtScl{\gwkHAT}{\wkm - \wkmhat} + \gamma^2 \SqrdNrm{\gwkHAT} \,.
\end{align*}

Taking expectation conditionally to $\wkm$, and using $\Expec{ \gwkHAT}{\wkm}= \Expec{\Expec{\gwkHAT}{\wkmhat}}{\wkm} =\Expec{\nabla F(\wkmhat)}{\wkm}$, we obtain:
\begin{align*}
    \Expec{\SqrdNrm{w_k - w_*}}{\wkm} &\leq \SqrdNrm{\wkm - w_*} - \Expec{2\gamma \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm} \\
    &\qquad- 2\gamma \Expec{\PdtScl{\nabla F (\wkmhat)}{\wkm - \wkmhat}}{\wkm} \\
    &\qquad+ \gamma^2 \Expec{\SqrdNrm{\gwkHAT}}{\wkm} \,.
\end{align*}

Then invoking \Cref{app:lem:grad_sto_to_grad} to upper bound the squared norm of the stochastic gradients, and noticing that $\Expec{\PdtScl{\nabla F(\wkm)}{\wkmhat-\wkm}}{\wkm}=0$ leads to:
\begin{align}
    \Expec{\SqrdNrm{w_k - w_*}}{\wkm} &\leq \SqrdNrm{\wkm - w_*} - 2\gamma\Expec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm} \nonumber \\
    &\quad - 2\gamma\Expec{ \PdtScl{\nabla F (\wkmhat) - \nabla F(\wkm)}{\wkm - \wkmhat}}{\wkm} \label{eq:decomp_heterog} \\
    &\quad + \gamma^2 \left( \bigpar{1 + \frac{4\omgC\up }{N}} L \Expec{\PdtScl{\nabla F(\wkmhat)}{\wkmhat - w_*}}{\wkmhat} \right.  \nonumber\\
    &\qquad \left.+ 2\omgC\up \Expec{\upMemTerm_{k-1}}{\wkmhat} + \frac{\sigma^2}{Nb} (1 + 4 \omgC\up) \right) \,. \nonumber
\end{align}


Now using Cauchy-Schwarz inequality (\cref{app:basic_ineq:cauchy_schwarz}) and smoothness: 
\begin{align*}
    &- \Expec{2\gamma \PdtScl{\nabla F (\wkmhat) - \nabla F(\wkm) }{\wkm - \wkmhat}}{\wkm} \\
    &\qqquad= 2\gamma \Expec{\PdtScl{\nabla F (\wkmhat) - \nabla F(\wkm)}{\wkmhat - \wkm}}{\wkm} \\
    &\qqquad\leq 2 \gamma L \Expec{\SqrdNrm{\wkmhat - \wkm}}{\wkm} \,,
\end{align*}

and thus:
\begin{align}
\label{app:eq:common_all_demo_convex}
\begin{split}
    \Expec{\SqrdNrm{w_k - w_*}}{\wkm} &\leq \SqrdNrm{\wkm - w_*} - 2\gamma\Expec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm} \\
    &\qquad + 2\gamma L \Expec{\SqrdNrm{\wkmhat - \wkm}}{\wkm} \\
    &\qquad + \bigpar{1 + \frac{4\omgC\up }{N}} \gamma^2 L \Expec{\PdtScl{\nabla F(\wkmhat)}{\wkmhat - w_*}}{\wkmhat}  \\
    &\qquad + 2\omgC\up \gamma^2 \Expec{\upMemTerm_{k-1}}{\wkmhat} + \frac{\sigma^2 \gamma^2 }{Nb} (1 + 4 \omgC\up) \,.
\end{split}
\end{align}

With \Cref{app:prop:ghost_variance_heterog}:
\begin{align*}
\begin{split}
    \Expec{\SqrdNrm{w_k - w_*}}{\wkm} &\leq \SqrdNrm{\wkm - w_*} - 2\gamma\Expec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm} \\
    &\qquad + 2\gamma^3 L^2\bigpar{1 + \frac{4\omgC\up }{N}} \omgC\dwn \Expec{\PdtScl{\nabla F(w_{k-2}}{w_{k-2} - w_*}}{w_{k-2}} \\
    &\qquad + 4\omgC\up \omgC\dwn \gamma^3L \Expec{\upMemTerm_{k-2}}{w_{k-2}} + \frac{\gamma^3 L \omgC\dwn \sigma^2}{Nb} (1 + 4 \omgC\up) \\
    &\qquad + \bigpar{1 + \frac{4\omgC\up }{N}} \gamma^2 L \Expec{\PdtScl{\nabla F(\wkmhat)}{\wkmhat - w_*}}{\wkmhat}  \\
    &\qquad + 2\omgC\up \gamma^2 \Expec{\upMemTerm_{k-1}}{\wkmhat} + \frac{\sigma^2 \gamma^2 }{Nb} (1 + 4 \omgC\up) \,.
\end{split}
\end{align*}

Reordering the terms and splitting in two the term $- 2\gamma\Expec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm}$ gives:
\begin{align}
\label{app:eq:ghost_before_build_lyapunov_heterog}
\begin{split}
    \Expec{\SqrdNrm{w_k - w_*}}{\wkm} &\leq \SqrdNrm{\wkm - w_*} - \gamma\Expec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm} \\
    &\qquad- \gamma \bigpar{ 1 - \gamma L \bigpar{1 + \ffrac{4 \omgC\up}{N} } } \Expec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm} \\
    &\qquad + 2\gamma^3 L^2\bigpar{1 + \frac{4\omgC\up }{N}} \omgC\dwn \Expec{\PdtScl{\nabla F(w_{k-2}}{w_{k-2} - w_*}}{w_{k-2}} \\
    &\qquad + 2\omgC\up \gamma^2\Expec{\upMemTerm_{k-1}}{\wkmhat} + 4\omgC\up \omgC\dwn \gamma^3L \Expec{\upMemTerm_{k-2}}{w_{k-2}} \\
    &\qquad+ \frac{\gamma^2 \sigma^2 (1+4\omgC\up)}{Nb} (1 + 2 \gamma L \omgC\dwn) \,.
\end{split}
\end{align}


Next, we use \Cref{app:lem:recursive_inequalities_over_memory} which corresponds to Lemma S13 of \citet{philippenko_artemis_2020} whose themselves get inspired from \citet{mishchenko_distributed_2019}
\begin{align}
\label{app:eq:recursive_inequalities_over_memory}
\begin{split}
    \Expec{\upMemTerm_{k}}{\wkm} &\leq (1 - \TOne) \Expec{\upMemTerm_{k-1}}{\wkm} \\
    &\qquad+ \ffrac{2\TTwo L}{N}\Expec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}{\wkm} \\
    &\qquad+  \frac{2}{N} \ffrac{\sigma^2}{b} \TTwo \,.
\end{split}
\end{align}

We take the full expectation (without conditioning over any random vectors) and we build a Lyapunov function with the two previous equation. However, observe that we use twice the \cref{app:eq:recursive_inequalities_over_memory} at step $k$ and $k-1$ in the Lyapunov: 
\begin{align*}
    V_k &= \FullExpec{\SqrdNrm{w_k - w_*}} + \ffrac{\gamma}{2}\FullExpec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}} +  \gamma^2 \cst_1 \FullExpec{\upMemTerm_{k-1}} + \gamma^3 L \cst_2 \FullExpec{\upMemTerm_{k-2}} \,,
\end{align*}
with $\cst_1 = \ffrac{2 \omgC\up}{\TTwo}$ and $\cst_2 = \ffrac{4 \omgC\dwn \omgC\up}{\TOne}$.

We combine as following
$(\ref{app:eq:ghost_before_build_lyapunov_heterog}) + \gamma^2 \cst_1 (\ref{app:eq:recursive_inequalities_over_memory})_{k} + \gamma^3 L \cst_2 (\ref{app:eq:recursive_inequalities_over_memory})_{k-1}$:
\begin{align*}
\begin{split}
    &\FullExpec{\SqrdNrm{w_k - w_*}} + \gamma \bigpar{ 1 - \gamma L \bigpar{1 + \ffrac{4 \omgC\up}{N} } } \FullExpec{\PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}\\ 
    &+\gamma^2 \cst_1 \FullExpec{\upMemTerm_{k}} + \gamma^3 L \cst_2 \FullExpec{\upMemTerm_{k-1}} \\
    &\qquad\leq \SqrdNrm{\wkm - w_*} - \gamma\FullExpec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}} \\
    &\qqquad + 2\gamma^3 L^2\bigpar{1 + \frac{4\omgC\up }{N}} \omgC\dwn \FullExpec{\PdtScl{\nabla F(w_{k-2}}{w_{k-2} - w_*}} \\
    &\qqquad + 2\omgC\up \gamma^2 \FullExpec{\upMemTerm_{k-1}} + 4\omgC\up \omgC\dwn \gamma^3L \FullExpec{\upMemTerm_{k-2}} \\
    &\qqquad +(1 - \TOne) \gamma^2\cst_1 \FullExpec{\upMemTerm_{k-1}} + \ffrac{2 \TTwo L\gamma^2 \cst_1}{N} \FullExpec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}} \\
    &\qqquad +(1 - \TOne) \gamma^3 L \cst_2 \FullExpec{\upMemTerm_{k-2}} + \ffrac{2 \TTwo \gamma^3 L^2 \cst_2}{N} \FullExpec{ \PdtScl{\nabla F (\widehat{w}_{k-2})}{\widehat{w}_{k-2} - w_*}} \\
    &\qqquad+ \frac{\gamma^2 \sigma^2 (1+4\omgC\up)}{Nb} (1 + 2 \gamma L \omgC\dwn) + \ffrac{2 \TTwo \gamma^2 \cst_1}{N^2} + \ffrac{2 \TTwo \gamma^3 L \cst_2}{N^2}
    \,,
\end{split}
\end{align*}

which is equivalent to:
\begin{align*}
\begin{split}
    &\FullExpec{\SqrdNrm{w_k - w_*}} + \gamma \bigpar{ 1 - \gamma L \bigpar{1 + \ffrac{4 \omgC\up}{N}  + \ffrac{2\TTwo \cst_1}{ N} } } \FullExpec{\PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}}\\ 
    &+\gamma^2 \cst_1 \FullExpec{\upMemTerm_{k}} + \gamma^3 L \cst_2 \FullExpec{\upMemTerm_{k-1}} \\
    &\qquad\leq \SqrdNrm{\wkm - w_*} - \gamma\FullExpec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}} \\
    &\qqquad + \bigpar{2\gamma^3 L^2\bigpar{1 + \frac{4\omgC\up }{N}} \omgC\dwn + \frac{2 \TTwo \gamma^3 L^2 \cst_2}{N} } \FullExpec{\PdtScl{\nabla F(w_{k-2}}{w_{k-2} - w_*}} \\
    &\qqquad + \bigpar{2\omgC\up \gamma^2 + (1 - \TOne) \gamma^2 \cst_1} \FullExpec{\upMemTerm_{k-1}} + \bigpar{4\omgC\up \omgC\dwn \gamma^3L + (1 - \TOne) \gamma^3 L \cst_2} \FullExpec{\upMemTerm_{k-2}} \\
    &\qqquad+ \frac{\gamma^2 \sigma^2}{Nb} \bigpar{ (1+4\omgC\up) (1 + 2 \gamma L \omgC\dwn) + 2 \TTwo \cst_1  + 2 \TTwo \gamma L \cst_2 }
    \,.
\end{split}
\end{align*}


To get contraction, we need to check each term of the Lyapunov function. First because $C_1 = \frac{2 \omgC\up}{\TOne}$, we have: 
$$
2\omgC\up + (1 - \TOne) \cst_1 = \cst_1 \,,
$$
and thus we obtain the contraction for the term $\FullExpec{\upMemTerm_{k-1}}$.

Secondly because $C_2 = 4 \omgC\dwn \omgC\up / \TOne$, the following condition is true:
\begin{align*}
    4\omgC\up \omgC\dwn \gamma^3L + (1 - \TOne) \gamma^3 L \cst_2 = 4\omgC\up \omgC\dwn \gamma^3L \bigpar{1 + \frac{1 - \TOne}{\TOne}} \leq \gamma^3 L \cst_2 = 4\omgC\up \omgC\dwn \gamma^3L \frac{1}{\TOne} \,.
\end{align*}


Furthermore, we need to handle the scalar product term. On the left hand side:
\begin{align*}
    &\gamma / 2 \leq \bigpar{1 - \gamma L \bigpar{1 + \ffrac{4 \omgC\up}{ N} + \ffrac{2\TTwo \cst_1}{N}} } \gamma \\
    \Longleftrightarrow \quad & \gamma L \bigpar{1 + \ffrac{4 \omgC\up}{ N} + \ffrac{2\TTwo \cst_1}{N}} \leq 1 /2
\end{align*}

We split this condition in two conditions and we consider that:
\[
\left\{
    \begin{array}{ll}
        1 + \ffrac{4 \omgC\up}{ N} \leq 1 / 4 \Longleftrightarrow \gamma L \leq \ffrac{1}{4 \bigpar{1 + \ffrac{4 \omgC\up}{ N}}} \\
        \ffrac{2\TTwo \cst_1}{N} \leq 1 / 4 \Longleftrightarrow \gamma L \leq \ffrac{N}{16 \omgC\up \TTwo}
    \end{array}
\right.
\]


Now, with the right hand side of the scalar product term we again split in two sub-conditions:
\[
\left\{
    \begin{array}{ll}
        2\gamma^3 L^2\bigpar{1 + \frac{4\omgC\up }{N}} \omgC\dwn \leq 1/4 \Longleftrightarrow \gamma L \leq \ffrac{1}{2 \sqrt{2 \omgC\dwn\bigpar{1 + \frac{4\omgC\up }{N}}}} \\
        \frac{2 \TTwo \gamma^3 L^2 \cst_2}{N} \leq \gamma /2 \Longleftrightarrow \gamma L \leq \ffrac{\sqrt{N }}{4\sqrt{2  \omgC\dwn \omgC\up}} \,.
    \end{array}
\right.
\]


Finally, we have:
\begin{align*}
\begin{split}
    &\FullExpec{\SqrdNrm{w_k - w_*}} + \ffrac{\gamma}{2} \FullExpec{\PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}} +\gamma^2 \cst_1 \FullExpec{\upMemTerm_{k}} + \gamma^3 L \cst_2 \FullExpec{\upMemTerm_{k-1}} \\
    &\qquad\leq \SqrdNrm{\wkm - w_*} - \gamma\FullExpec{ \PdtScl{\nabla F (\wkmhat)}{\wkmhat - w_*}} \\
    &\qqquad + \ffrac{1\gamma}{2} \FullExpec{\PdtScl{\nabla F(w_{k-2}}{w_{k-2} - w_*}} \\
    &\qqquad + \gamma^2 \cst_1 \FullExpec{\upMemTerm_{k-1}} + \gamma^3 L \cst_2\FullExpec{\upMemTerm_{k-2}} \\
    &\qqquad+ \frac{\gamma^2 \sigma^2}{Nb} \bigpar{ (1+4\omgC\up) (1 + 2 \gamma L \omgC\dwn) + 4 \omgC\up  \bigpar{1 + 2 \gamma L \omgC\dwn }}
    \,.
\end{split}
\end{align*}

Applying convexity with \cref{app:ineq_convex_demi_and_demi}:
\begin{align*}
V_k \leq V_{k-1} - \gamma \FullExpec{F(\wkm) - F(w_*)} + \frac{\gamma^2 \sigma^2 \Phi^{\Gheterog}(\gamma)}{Nb}\,,
\end{align*}
with $\Phi^{\Gheterog}(\gamma) := \bigpar{1+8\omgC\up } \bigpar{1 + 2 \gamma L \omgC\dwn} $.

Invoking Jensen inequality (\ref{app:basic_ineq:jensen}) leads to $\FullExpec{F(\wkmhat)}\geq \FullExpec{F(\wkm)}$, we finally obtain:
\begin{align*}
V_k \leq V_{k-1} - \gamma \FullExpec{F(w_{k-1}) - F(w_*)} + \frac{\gamma^2 \sigma^2 \Phi^{\Gheterog}(\gamma)}{Nb}\,.
\end{align*}

\end{proof}

==> style/preambule.tex <==
\PassOptionsToPackage{numbers}{natbib}
\bibliographystyle{plainnat}

\usepackage[final]{style/neurips_2021}


\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\RequirePackage[colorlinks,allcolors=blue]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{hyperref}

\usepackage{stmaryrd} % For double bracket 
\usepackage{amsthm}
\usepackage{thmtools, thm-restate} % for proofs in appendix
\usepackage[normalem]{ulem} % for command \sout. normalem => because ulem transform emphatise and we want to switch off this feature.
\usepackage{mdframed} % hightlight env with background color
\usepackage{multirow} % to merge cell on same column in a table

\usepackage{amsmath}
\usepackage{amssymb} 

\usepackage{float}
\usepackage{subcaption} % for picture side-by-side

\usepackage{cleveref} %for \Cref

\usepackage{booktabs} % for multicolumns
\usepackage{colortbl} % for \rowcolor{green!25}

\usepackage{vwcol} % to wrap fig inside text.


\usepackage{pifont} %For checkmark and cross
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\usepackage[dvipsnames]{xcolor} %for extended colors
\usepackage{multicol}

\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{graphicx}
\graphicspath{{pictures/}} %Setting the graphicspath

\usepackage{enumitem}

\usepackage{wrapfig}
\usepackage{tocloft}


% For code
\usepackage{xcolor}

% For shaded theorems
\usepackage{xcolor}
\usepackage{framed}
\theoremstyle{plain}

% Defining flowchart with tikz
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}
\tikzstyle{centralserver} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=red!30]
\tikzstyle{nodeserver} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
\usetikzlibrary{automata,positioning}
\usepackage{makecell}

% For note in latex
\usepackage{xargs} 

\title{Preserved central model for faster bidirectional compression in distributed settings}

\author{
  Constantin Philippenko \quad Aymeric Dieuleveut \\
  CMAP, École Polytechnique, Institut Polytechnique de Paris\\
  \texttt{[fistname].[lastname]@polytechnique.edu} \\
}






==> table_comparison_bi_algo.tex <==

\begin{table*}
\caption{\label{table:comparison_algo_bi}Comparison of frameworks for main algorithms handling bidirectional compression. By ``non i.i.d.'',~we mean that the theoretical framework encompasses \textit{and} explicitly quantifies the impact of data heterogeneity on convergence (\Cref{asu:bounded_noises_across_devices}), e.g., \texttt{Dore} does not assume i.i.d.~workers but does not quantify differences between distributions.}
\centering
\begin{tabular}{lccccc}
 \hline
  & \thead{
  \texttt{Dore} 
  \\ \cite{liu_double_2020}}
  & \thead{\texttt{Double} \\ \texttt{Squeeze} \\
  \cite{tang_doublesqueeze_2019}} 
  & \thead{\texttt{Dist} \\ \texttt{EF-SGD}
  \\ \cite{zheng_communication-efficient_2019}} 
  & \thead{\Artemis \\ \cite{philippenko_artemis_2020}} 
  & \thead{\texttt{STC} \\ \cite{sattler_robust_2019}} \\
  \hline
  Data & i.i.d.& i.i.d. &i.i.d. & \textcolor{ForestGreen}{non i.i.d.} \\
  Bounded variance&\thead{\textcolor{red}{Uniformly}}&\thead{\textcolor{red}{Uniformly}}&\thead{\textcolor{red}{Uniformly}}&\thead{\textcolor{ForestGreen}{At optimal} \\ 
  \textcolor{ForestGreen}{point}} \\
  Error compensation &\cmark&\cmark&\cmark& \\
  Memory &\cmark&&&\cmark \\
  \hline
\end{tabular}%}
\gs\gs
\end{table*}
